Adaptive Reduced Basis Methods for Multiscale Problems and Large-scale PDE-constrained Optimization

This thesis presents recent advances in model order reduction methods with the primary aim to construct online-efficient reduced surrogate models for parameterized multiscale phenomena and accelerate large-scale PDE-constrained parameter optimization methods. In particular, we present several different adaptive RB approaches that can be used in an error-aware trust-region framework for progressive construction of a surrogate model used during a certified outer optimization loop. In addition, we elaborate on several different enhancements for the trust-region reduced basis (TR-RB) algorithm and generalize it for parameter constraints. Thanks to the a posteriori error estimation of the reduced model, the resulting algorithm can be considered certified with respect to the high-fidelity model. Moreover, we use the first-optimize-then-discretize approach in order to take maximum advantage of the underlying optimality system of the problem. In the first part of this thesis, the theory is based on global RB techniques that use an accurate FEM discretization as the high-fidelity model. In the second part, we focus on localized model order reduction methods and develop a novel online efficient reduced model for the localized orthogonal decomposition (LOD) multiscale method. The reduced model is internally based on a two-scale formulation of the LOD and, in particular, is independent of the coarse and fine discretization of the LOD. The last part of this thesis is devoted to combining both results on TR-RB methods and localized RB approaches for the LOD. To this end, we present an algorithm that uses adaptive localized reduced basis methods in the framework of a trust-region localized reduced basis (TR-LRB) algorithm. The basic ideas from the TR-RB are followed, but FEM evaluations of the involved systems are entirely avoided.

==> frontmatter/titlepages_ulb_version.tex <==
% title page
\begin{titlepage}
\centering

~\vspace{10\baselineskip}

{\Large
MATHEMATIK\par}
% Fach: Mathematik\par}
\vspace{2\baselineskip}

{\Huge \bfseries
	Model reduction for kinetic equations: moment approximations and hierarchical approximate proper orthogonal decomposition\par}
%\vspace{8\baselineskip}
\vfill

{\large
Inauguraldissertation \\
zur Erlangung des Doktorgrades der Naturwissenschaften \\
im Fachbereich Mathematik und Informatik \\
der Mathematisch-Naturwissenschaftlichen Fakultät \\
der Westfälischen Wilhelms-Universität Münster
\par}
\vspace{4\baselineskip}


{\large
vorgelegt von \\
Tobias Leibner \\
aus Osnabrück
\par
}
% \medskip

% {\Large
% }
% \medskip

% {\Large
% }
\vspace{2\baselineskip}

{\large
- 2021 - % chktex 8
}


\end{titlepage}

% cspell: disable
% back of title page
\thispagestyle{empty}
\par\vspace*{\fill}
%
{\textcolor{Gray}\hrule}
%
~\\[\baselineskip]
%
\textbf{Dekan:} Prof.\ Dr.\ Xiaoyi Jiang \\
\textbf{Erstgutachter:} Prof.\ Dr.\ Mario Ohlberger \\
\textbf{Zweitgutachter:} Prof.\ Dr.\ Axel Klar\\
%
~\\
%
\textbf{Tag der mündlichen Prüfung:}\hspace{1cm}
\begin{minipage}[t]{5cm}
	% gepunktete Linie
	\centering \dotfill \\
	% Text unter der Linie
	\end{minipage} \\
\textbf{Tag der Promotion:}
\hspace{2.721cm} \begin{minipage}[t]{5cm}
	% gepunktete Linie
	\centering \dotfill \\
	% Text unter der Linie
	\end{minipage}


==> pagestyle.tex <==
% cspell: disable
% \pagestyle{fancyplain}

% \setlength{\headheight}{15 pt}                                          %%setzt die Größe der Kopfzeile fest
% \setlength{\textheight}{230 mm}                                         %%setzt die Länge des Textrumpfes fest
% \setlength{\parindent}{0em}                                                     %%verhindert das Einrücken am Anfang eines neuen Absatzes
% \setlength{\parskip}{6pt}                            %% Abstand nach Absatz

% \pagestyle{fancyplain}
% \renewcommand{\sectionmark}[1]{\markboth{#1}{}}                         %%soll das Kapitel oben in der Kopfzeile ohne Nummer anzeigen und verhindert Konvertierung in uppercase

% \lhead{\fancyplain{}{\textit{\leftmark}}}       %Seitenlayout
% \chead{}
% \rhead{\fancyplain{}{\thepage}}
% \lfoot{}
% \cfoot{}
% \rfoot{}
% \onehalfspacing % chktex 1
% \abovedisplayskip=7pt plus 3pt minus 4pt
% \abovedisplayshortskip=0pt plus 3pt
% \belowdisplayskip=7pt plus 3pt minus 4pt
% \belowdisplayshortskip=4pt plus 3pt minus 4pt

%% abstände vor und nach sections ändern
% \makeatletter
% \renewcommand\subsection{\@startsection % chktex 1
%    {subsection}{2}{0mm}%      % name, ebene, einzug
%    {\baselineskip}%            % vor-abstand
%    {0.1\baselineskip}%            % nach-abstand
%    {\bfseries\large}%           % layout
% }
% \makeatother

% \makeatletter
% \renewcommand\subsubsection{\@startsection % chktex 1
%    {subsubsection}{3}{0mm}%      % name, ebene, einzug
%    {\baselineskip}%            % vor-abstand
%    {0.1\baselineskip}%            % nach-abstand
%    {\bfseries\normalsize}%           % layout
% }
% \makeatother

% \setlength\partopsep{-0.3\topsep} %% um den abstand zwischen c++ code in minted umgebungen und text zu verkleinern

